An Uncertainty Principle for Linear Recurrent Neural Networks

We consider linear recurrent neural networks, which have become a key building block of sequence modeling due to their ability for stable and effective long-range modeling. In this paper, we aim at characterizing this ability on a simple but core copy task, whose goal is to build a linear filter of order $S$ that approximates the filter that looks $K$ time steps in the past (which we refer to as the shift-$K$ filter), where $K$ is larger than $S$. Using classical signal models and quadratic cost, we fully characterize the problem by providing lower bounds of approximation, as well as explicit filters that achieve this lower bound up to constants. The optimal performance highlights an uncertainty principle: the optimal filter has to average values around the $K$-th time step in the past with a range~(width) that is proportional to $K/S$.

==> sections/storage_for_modifs.tex <==
\begin{definition}[Discrete-Time Fourier Transform]
    For a discrete-time sequence $(u_n)_n$, the discrete-time Fourier transform is, for $\omega\in[0, 2\pi]$,
    \begin{equation}
          U(e^{j\omega})=\sum_{n=-\infty}^\infty u_ne^{-j\omega n}  
    \label{DTFT}
    \end{equation}

    and its inverse Fourier transform 
    \begin{equation}
    u_n = \frac{1}{2\pi}\int_{-\pi}^\pi U(e^{j\omega})e^{j\omega n}d\omega
    \label{inverse DTFT}
    \end{equation}
    
\end{definition}

The \textit{z-Transform} is a generalization of the discrete-time Fourier transform, extending it to complex values of \(z\), whereas the Fourier transform is obtained by evaluating the \textit{z-transform} on the unit circle.


\begin{definition}[z-Transform]
    Given a sequence $(u_n)_n$, for a complex number $z$, the \textit{z-transform} is 
    \begin{equation}
    U(z) = \sum_{n=-\infty}^\infty u_nz^{-n}
    \label{Z-transform}
    \end{equation}
    Comparing \ref{DTFT} and \ref{Z-transform}, the Fourier-transform can be obtained evaluating the \textit{z-Transform} at the unit circle.
\end{definition}
The \textit{z-transform} satisfies the shifting property: if \( (u_n) \) is a discrete-time signal and \( \tau \in \mathbb{Z} \), the shifted signal \( (v_n) = (u_{n-\tau}) \) has the z-transform \( V(z) = z^{-\tau} U(z) \). This property allows to compute the transfer function of a signal defined by difference equations.
\\

We recall Parseval's theorem that establishes a fundamental equivalence between the inner product of two signals in the time domain and their corresponding representation in the frequency domain.

\begin{definition}[Parseval's theorem]
    For two complex-valued discrete-time signals \(x_n\) and \(y_n\) with discrete-time Fourier transforms \(X(e^{j\omega})\) and \(Y(e^{j\omega})\), Parseval's theorem yields:
    \begin{equation}
        \sum_{n=-\infty}^{+\infty}x_n\overline{y_n} = \frac{1}{2\pi}\int_0^{2\pi}X(e^{j\omega})\overline{Y(e^{j\omega})}d\omega
        \label{Parseval thm}
    \end{equation}
In particular, Parseval's theorem yields an energy conservation result:
    \begin{equation*}
        \sum_{n=-\infty}^{+\infty}\vert x_n\vert^2 = \frac{1}{2\pi}\int_0^{2\pi}\vert X(e^{j\omega})\vert^2 d\omega
    \end{equation*}

\end{definition}


Applying the \textit{z-transform} to the difference equation \ref{Difference equation} allows us to compute the transfer function of a linear time-invariant (LTI) system, i.e., the \textit{z-transform} of the impulse response \( (c_n) \) as shown in \ref{LTI convolution filter}. The transfer function \( C(z) \) characterizes the system's input-output relationship and is given by the ratio of the z-transforms of the output and input:
\[
C(z) = \frac{X(z)}{U(z)} = \frac{\sum_{k=0}^S h_k z^{-k}}{\sum_{k=0}^S g_k z^{-k}},
\]
where \( g_0 = 1 \). It can be further decomposed using partial fraction decomposition:
\begin{equation}
C(z) = \sum_{s=-S/2}^{S/2} \frac{b_s}{1 - a_s z^{-1}},
\label{Partial fraction decomposition}
\end{equation}

where \( (a_s) \) are complex numbers with modulus less than 1, and \( (b_s) \) are coefficients. 

The Fourier transform of the impulse response, \( C(e^{j\omega}) \), can be obtained by evaluating the transfer function on the unit circle. This will be of particular relevance later in the paper.

\paragraph{First Case: $\epsilon > 1$} \\
Let us define, for $u \in \mathbb{N}$ and $\alpha > 0$, 
\[
\phi_u(\alpha) = \frac{(-1)^u}{\alpha - i\pi u}.
\]
For any $\alpha > 0$, the series 
\[
\sum_{u=-\infty}^{+\infty} \phi_u(\alpha)
\]
is an alternating series whose general term decreases to 0 in norm. Moreover, the sequence of functions $(\phi_u)_u$ uniformly decreases to 0 on $[0.1, 10]$. Thus, the series of functions $\sum_{u=-\infty}^{+\infty} \phi_u$ converges uniformly on $[0.1, 10]$. 

Now, consider the sum $\sum_{u=-S}^S \frac{e^{i\pi u}}{\alpha - i\pi(u + \epsilon S)}$ for $\alpha \in [\pi, 10]$. Take $\delta > 0$ and $N \in \mathbb{N}$ such that for any $\alpha$ with $\vert\alpha\vert \in [0.1, 10]$, 
\[
\left| \sum_{u=N}^{+\infty} \phi_u(\alpha) \right| \leq \frac{\delta}{2}.
\]
Decompose $\epsilon$ as $\epsilon = \frac{n}{S} + \frac{\beta}{S}$, where $n = \lfloor \epsilon S \rfloor \in \llbracket S+1, +\infty \rrbracket$ and $\beta \in [0,1]$. We then write:
\begin{align*}
    \sum_{u=-S}^S \frac{e^{i\pi u}}{\alpha - i\pi(u + \epsilon S)} 
    &= \sum_{u=-S}^S \frac{e^{i\pi u}}{\alpha - i\pi(u + n + \beta)} \\
    &= \sum_{u=-S+n}^{S+n} \frac{e^{i\pi u}}{\tilde{\alpha} - i\pi u}, \quad \text{with } \tilde{\alpha} = \alpha - i\pi \beta.
\end{align*}
We have $\vert \tilde{\alpha} \vert > 0.1$, and as $S \to +\infty$, $-S+n \to +\infty$. For $S$ such that $-S+n > N$, we find:
\begin{align*}
    \left| \sum_{u=-S}^S \frac{e^{i\pi u}}{\alpha - i\pi(u + \epsilon S)} \right| 
    &= \left| \sum_{u=-S+n}^{+\infty} \frac{e^{i\pi u}}{\tilde{\alpha} - i\pi u} - \sum_{u=S+n}^{+\infty} \frac{e^{i\pi u}}{\tilde{\alpha} - i\pi u} \right| \\
    &\leq \frac{\delta}{2} + \frac{\delta}{2} = \delta.
\end{align*}

\paragraph{Second Case: $\epsilon < 1$} \\
Consider the sum $\sum_{u=-S}^S \frac{e^{i\pi u}}{\alpha - i\pi(u + \epsilon S)}$. Decompose $\epsilon$ as $\epsilon = \frac{n}{S} + \frac{\beta}{S}$, where $n = \lfloor \epsilon S \rfloor \in \llbracket -S, S \rrbracket$ and $\beta \in [0,1]$. We then write:
\begin{align*}
    \sum_{u=-S}^S \frac{e^{i\pi u}}{\alpha - i\pi(u + \epsilon S)} 
    &= \sum_{u=-S}^S \frac{e^{i\pi u}}{\alpha - i\pi(u + n + \beta)} \\
    &= \sum_{u=-S+\lfloor \epsilon S \rfloor}^{S+\lfloor \epsilon S \rfloor} \frac{e^{i\pi u}(-1)^{\lfloor \epsilon S \rfloor}}{\tilde{\alpha} - i\pi u}, \quad \text{with } \tilde{\alpha} = \alpha - i\pi \beta.
\end{align*}
We study the limit as $S \to +\infty$:
\begin{align*}
    \lim_{S \to +\infty} \sum_{u=-S+\lfloor \epsilon S \rfloor}^{S+\lfloor \epsilon S \rfloor} \frac{e^{i\pi u}}{\tilde{\alpha} - i\pi u}
    &= \lim_{S \to +\infty} \left( \sum_{u=-S+n}^{S-n} \frac{(-1)^u}{\tilde{\alpha} - i\pi u} + \sum_{u=S-n+1}^{S+n} \frac{(-1)^u}{\tilde{\alpha} - i\pi u} \right).
\end{align*}
For fixed $\epsilon$, the series $\sum_{u=-\infty}^{+\infty} \frac{(-1)^u}{\alpha - i\pi u}$ converges uniformly with respect to $\alpha$. Thus, even though $\tilde{\alpha}$ depends on $S$, 
\[
\lim_{S \to +\infty} \sum_{u=S-n+1}^{S+n} \frac{(-1)^u}{\tilde{\alpha} - i\pi u} = 0.
\]
We are left with:
\[
\lim_{S \to +\infty} \sum_{u=-S+n}^{S-n} \frac{(-1)^u}{\tilde{\alpha} - i\pi u}.
\]
Since $\tilde{\alpha} = \alpha - i\pi \beta$ does not converge to a fixed value as $S \to +\infty$, for large $S$, we approximate:
\begin{align*}
    \sum_{u=-S+n}^{S-n} \frac{(-1)^u}{\tilde{\alpha} - i\pi u} &\approx \frac{2}{e^{\tilde{\alpha}} - e^{-\tilde{\alpha}}} \\
    &= \frac{2}{e^{\alpha}e^{i\pi \beta} - e^{-\alpha}e^{-i\pi \beta}}, \quad \text{with } \beta = \epsilon S - \lfloor \epsilon S \rfloor.
\end{align*}



\subsection{z-Transforms and Transfer Function}

\paragraph{z-Transform}  
For a complex number \(z = re^{j\phi}\), the z-transform of a discrete-time signal \(x[n]\) is defined as:
\begin{equation}
X(z) = \sum_{n=-\infty}^{+\infty} x[n] z^{-n}, \label{appendix z-transform}
\end{equation}
where \(z\) represents a point in the complex plane. The inverse z-transform is given by:
\[
x[n] = \frac{1}{2\pi \mathrm{i}} \oint X(z) z^{n-1} \, dz,
\]
where the integration is performed along a closed contour within the region of convergence (ROC).  

The relationship between \(x[n]\) and \(X(z)\) is denoted as:
\[
x[n] \overset{z}{\longleftrightarrow} X(z).
\]

The z-transform exists if the infinite sum in \eqref{appendix z-transform} converges. A necessary condition for convergence is the absolute summability of \(x[n]z^{-n}\). Since \(\vert x[n]z^{-n}\vert = \vert x[n]r^{-n} \vert\), the condition becomes:
\[
\sum_{n=-\infty}^{+\infty} \vert x[n] r^{-n} \vert < \infty.
\]
The range of \(r\) for which this condition holds is called the region of convergence (ROC).

Unlike the discrete-time Fourier transform (DTFT), the z-transform exists for certain signals that do not have a DTFT. For any signal \(x[n]\), the DTFT can be obtained by evaluating the z-transform at \(z = e^{j\omega}\).

\paragraph{Properties of the z-Transform}  
The z-transform has several useful properties:
\begin{itemize}
    \item \textit{Time Shift}: \(x[n-n_0] \overset{z}{\longleftrightarrow} z^{-n_0} X(z)\)
    \item \textit{Time Reversal}: \(x[-n] \overset{z}{\longleftrightarrow} X\left(\frac{1}{z}\right)\)
    \item \textit{Convolution}: \(x[n] \ast y[n] \overset{z}{\longleftrightarrow} X(z) Y(z)\)
\end{itemize}

\paragraph{Transfer Function}  
Consider applying the input \(x[n] = z^n\) to a linear time-invariant (LTI) system with impulse response \(h[n]\). The system output \(y[n]\) is given by the convolution of \(h[n]\) and \(x[n]\):
\[
y[n] = h[n] \ast x[n] = \sum_{k=-\infty}^{+\infty} h[k] x[n-k].
\]

Substituting \(x[n] = z^n\) into this expression yields:
\[
y[n] = z^n \left( \sum_{k=-\infty}^{+\infty} h[k] z^{-k} \right).
\]

The transfer function \(H(z)\) is then defined as the z-transform of the system's impulse response \(h[n]\):
\begin{equation}
H(z) = \sum_{k=-\infty}^{+\infty} h[k] z^{-k}. \label{appendix transfer function}
\end{equation}

Thus, the system response to an input \(x[n] = z^n\) is characterized by:
\[
y[n] = H(z) z^n,
\]
where \(H(z)\) encapsulates the system's frequency response in the z-domain.

\paragraph{Transfer Function of an LTI System}  
For a linear time-invariant (LTI) system described by its impulse response \(h[n]\) and input \(x[n]\) via the convolution:
\[
y[n] = h[n] \ast x[n],
\]
the convolution property of the z-transform allows the transformed output \(Y(z)\) to be expressed as the product of the system's transfer function \(H(z)\) and the transformed input \(X(z)\):
\[
Y(z) = H(z) X(z).
\]
This implies that the transfer function can also be defined as the ratio of the z-transform of the output to that of the input:
\[
H(z) = \frac{Y(z)}{X(z)},
\]
where this relationship holds for all \(z\) such that \(X(z) \neq 0\).

The transfer function can be derived directly from the system's difference equation. For an LTI system described by:
\[
\sum_{k=0}^N h_k y[n-k] = \sum_{k=0}^M g_k x[n-k],
\]
applying the time-shift property of the z-transform to \(y[n]\) and \(x[n]\) yields:
\begin{equation}
H(z) = \frac{\sum_{k=0}^M g_k z^{-k}}{\sum_{k=0}^N h_k z^{-k}},
\label{appendix rational TF}
\end{equation}
where \(H(z)\) is a rational transfer function.

The numerator and denominator polynomials in \eqref{appendix rational TF} can be factorized as:
\[
H(z) = \frac{\Tilde{b} z^{-p} \prod_{k=1}^{M-p} (1 - c_k z^{-1})}{z^{-l} \prod_{k=1}^{N-l} (1 - a_k z^{-1})},
\]
where \(\Tilde{b} = b_p / a_l\) is the gain of the system, and \(c_k\) and \(a_k\) are the zeros and poles, respectively. These provide significant insights into the system's characteristics, particularly regarding stability and causality.  

- \textit{Poles and Stability}: A pole located inside the unit circle in the \(z\)-plane (\(\vert a_k \vert < 1\)) contributes an exponentially decaying term to the impulse response, while a pole located outside the unit circle (\(\vert a_k \vert > 1\)) contributes an exponentially growing term. Therefore, for a system to be stable, all its poles must lie strictly inside the unit circle.

The transfer function can also be expressed using partial fraction decomposition:
\begin{equation}
H(z) = \sum_{k=0}^r \frac{b_k}{1 - a_k z^{-1}},
\label{appendix partial fraction decomposition}
\end{equation}
where the poles \(a_k\) determine the system's stability and causality.

In summary, the transfer function encapsulates the system's behavior in the \(z\)-domain, with its poles and zeros providing critical information about the system's dynamic characteristics.




\subsection{A few signal processing tools}

\begin{definition}[Discrete-Time Fourier Transform]
    For a discrete-time sequence $(u_n)$, the discrete-time Fourier transform is, for $\omega\in[0, 2\pi]$,
    \begin{equation}
          U(e^{i\omega})=\sum_{n=-\infty}^\infty u_ne^{-i\omega n}  
    \label{DTFT}
    \end{equation}

    and its inverse Fourier transform 
    \begin{equation}
    u_n = \frac{1}{2\pi}\int_{-\pi}^\pi U(e^{i\omega})e^{i\omega n}d\omega
    \label{inverse DTFT}
    \end{equation}
    
\end{definition}

We recall Parseval's theorem that establishes a fundamental equivalence between the inner product of two signals in the time domain and their corresponding representation in the frequency domain.

\begin{definition}[Parseval's theorem]
    For two complex-valued discrete-time signals \((x_n)\) and \((y_n)\) with discrete-time Fourier transforms \(X(e^{i\omega})\) and \(Y(e^{i\omega})\), Parseval's theorem yields:
    \begin{equation}
        \sum_{n=-\infty}^{+\infty}x_n\overline{y_n} = \frac{1}{2\pi}\int_0^{2\pi}X(e^{i\omega})\overline{Y(e^{i\omega})}d\omega
        \label{Parseval thm}
    \end{equation}
In particular, Parseval's theorem yields an energy conservation result:
    \begin{equation*}
        \sum_{n=-\infty}^{+\infty}\vert x_n\vert^2 = \frac{1}{2\pi}\int_0^{2\pi}\vert X(e^{i\omega})\vert^2 d\omega
    \end{equation*}
\end{definition}

These definitions allow us to transform the time-domain loss \eqref{Time domain loss} into a frequency-domain loss:

\begin{theorem}\label{theorem frequency loss}
    Let \((c_n)=(c_k)_{k \geq 0}\) and \((d_n)=(d_k)_{k \geq 0}\) be discrete-time filters such that \(d_k=1_{k=K}\) and \(c_k=\sum_{s=1}^Sa_s^kb_s\) is its approximation with a linear recurrence of order \(S\). Let \(\gamma : \mathbb{Z} \to \mathbb{R}\) define the autocorrelation such that \(\gamma(k)=\rho^{\vert k\vert}\) for \(\rho > 0\). The approximation error is given by
\begin{equation}
\sum_{k, k'} (c_k - d_k)(c_{k'} - d_{k'}) \gamma(k - k') = \frac{1}{2\pi} \int_{-\pi}^\pi \bigg\vert\sum_{s=1}^{S}\frac{b_s}{1-a_se^{-i\omega}} - e^{-iK\omega}\bigg\vert^2 \Gamma(e^{i\omega}) d\omega
\label{Frequential loss copy task}
\end{equation}
where \(\Gamma(e^{i\omega})\) denotes the discrete-time Fourier transform of the autocorrelation factor \(\gamma\).
\end{theorem}

\begin{proof}
    Denoting \(C(e^{i\omega})\) and \(D(e^{i\omega})\) as the Fourier transforms of \((c_n)\) and \((d_n)\), respectively, Parseval's theorem gives:
    \[
    \sum_{k, k'} (c_k - d_k)(c_{k'} - d_{k'}) \gamma(k - k') = \frac{1}{2\pi} \int_{-\pi}^\pi \bigg\vert C(e^{i\omega}) - D(e^{i\omega})\bigg\vert^2 \Gamma(e^{i\omega}) d\omega.
    \]
    The Fourier transform of \((d_n)\) is \(D(e^{i\omega})=e^{-iK\omega}\). The Fourier transform \(C(e^{i\omega})\) of \((c_n)\) is given by 
    \[
    C(\omega) = \sum_{s=1}^S b_s \sum_{k=-\infty}^\infty \left(a_s e^{-i\omega}\right)^k = \sum_{s=1}^S \frac{b_s}{1 - a_s e^{-i\omega}}.
    \]
\end{proof}

Note that by developing this frequency loss, we come back to \eqref{Time domain loss}. We just transformed the time-domain problem into an complex approximation problem in the frequency space. This representation simply motivates the following parametrization. In a first time, we place ourselves in the white noise case, which is easier to analyze. We extend the results in a second time, showing that they hold in the autocorrelated case.


\begin{proof} \francis{not needed. We are not giving a class, just recalling the basics.}
    Consider the product of a signal $(x_n)$ and the impulse sequence $e_n$, written as 
    \[
    x_ne_n = x_0e_n
    \]
    Generalize this relationship to the product of $(x_n)$ and the time-shifted impulse sequence to obtain 
    \[
    x_ne_{n-k} = x_ke_{n-k}
    \]
    This property allows us to express $(x_n)$ as the following weighted sum of time-shifted impulses:
    \[
    x_n = \sum_{k=-\infty}^{+\infty}x_ke_{n-k}
    \]
    Now use the linearity property to interchange the system operator $H$ with the summation and signal values $x[k]$ to obtain 
    \begin{align*}
        y_n &= \sum_{k=-\infty}^{+\infty}x_kH\{e_{n-k}\}\\
        &=\sum_{k=-\infty}^{+\infty}x_kh_{n-k}
    \end{align*}
\end{proof}

An LTI system is bounded if $\sum_{k=-\infty}^{+\infty}\vert h_k\vert < \infty$ \francis{ is this needed?}

\begin{proof} \francis{ is this needed?}
    Let $x_n$ be a bounded input signal: $\vert x_n \leq M_x < \infty$. The magnitude of the output is given by 
    \begin{align*}
        \vert y_n\vert &= \vert h_n\ast x_n\vert\\
        &=\big\vert \sum_{k=-\infty}^\infty h_kx_{n-k}\big\vert\\
        &\leq \sum_{k=-\infty}^\infty\vert h_k\vert \vert x_{n-k}\vert\\
        &\leq M_x\sum_{k=-\infty}^\infty\vert h_k\vert
    \end{align*}
    Therefore, if $h_n$ is summable, $y_n$ is bounded for every bounded input $x_n$. 
\end{proof}

\subsubsection{Difference equations}
\francis{ is this needed?}
Linear constant-coefficients difference equations provide another way to represent the input-output characteristics of LTI in the time domain. Such an equation has the following form:
\[
\sum_{k=0}^N h_ky_{n-k} = \sum_{k=0}^M g_kx_{n-k}
\]
The integer $N$ is termed the order of the difference equation and corresponds to the maximum memory involving the system output. It represents the number of energy storage devices in the system. 


\begin{align*}
    (b_u) &= (C^{-1}\bar{a}^K)_u\\
    &= \big(\frac{M^{-1}}{K}\bar{a}^K\big)_u + \big[\big( C^{-1} - \frac{M^{-1}}{K}\big)\bar{a}^K\big]_u\\
    &= \big(\frac{M^{-1}_{\infty}}{K}\bar{a}_\infty^K\big)_u + \frac{1}{K}\big[\big(M^{-1}\bar{a}^K\big)_u - \big(M^{-1}_\infty \bar{a}_\infty^K\big)_u\big] + \big[\big( C^{-1} - \frac{M^{-1}}{K}\big)\bar{a}^K\big]_u.
\end{align*}

First, according to Lemma \ref{lemma eigenvector Toeplitz},
\[
\big(\frac{M^{-1}_{\infty}}{K}\bar{a}_\infty^K\big)_s= \frac{e^{-\alpha}(e^{2\alpha} - e^{-2\alpha})}{2K}(-1)^s.
\]

Second, \alex{i cant bound this because I struggle to express $M^{-1}$ wrt $M$}

Third, \begin{align*}
    \big\vert\big[\big( C^{-1} - \frac{M^{-1}}{K}\big)\bar{a}^K\big]_u\big\vert^2    &=\big\vert\big[\big(-C^{-1}(C - KM)\frac{M^{-1}}{K}\big)\bar{a}^K\big]_u\big\vert^2\\
    &\leq e^{-\alpha}\cdot\| C^{-1}\|^2\cdot\|\frac{M^{-1}}{K}\|^2\| C-KM\|^2\\
    &= e^{-\alpha}\frac{\kappa_2(C)}{\| C\|^2}\cdot\frac{\kappa_2(M)}{K\| M\|^2}\cdot\| C - KM\|^2.
\end{align*}

First, we bound $\| C-KM\|^2$.
\begin{align*}
    \| C - KM\|^2 &= \sum_{s, s'}\big\vert\frac{1}{1-e^{-2\alpha/K}e^{i(s-s')\pi/K}} - \frac{K}{2\alpha - i(s-s')\pi}\big\vert^2\\
    &= \sum_{s, s'}\big\vert \frac{2\alpha -i(s-s')\pi - K(1 - e^{-2\alpha/K}e^{i(s-s')\pi/K})}{(1-e^{-2\alpha/K}e^{i(s-s')\pi/K})(2\alpha - i(s-s')\pi)}\big\vert^2\\
    &= \sum_{s, s'}\big\vert\frac{2\alpha - i(s-s')\pi - K\big[\frac{2\alpha}{K} -i\frac{(s-s')\pi}{K} + \frac{1}{2}\big(\frac{4\alpha^2}{K^2} - \frac{(s-s')^2\pi^2}{K^2} -\frac{4i\pi\alpha(s-s')}{K^2} + o(\frac{1}{K^2})\big)\big]}{(1-e^{-2\alpha/K}e^{i(s-s')\pi/K})(2\alpha - i(s-s')\pi)}\big\vert^2\\
    &=\sum_{s, s'}\big\vert\frac{\frac{2\alpha^2}{K} - \frac{\pi^2(s-s')^2}{2K} - \frac{2i\pi\alpha(s-s')}{K} + o(\frac{1}{K})}{(1-e^{-2\alpha/K}e^{i(s-s')\pi/K})(2\alpha - i(s-s')\pi)}\big\vert^2\\
    &=\frac{1}{K^2}\sum_{s, s'}\big\vert\frac{2\alpha^2 - \frac{\pi^2(s-s')^2}{2} - 2i\pi\alpha(s-s') + o(1)}{(1-e^{-2\alpha/K}e^{i(s-s')\pi/K})(2\alpha - i(s-s')\pi)}\big\vert^2\\
    &= O\big(T^2\big). \text{\alex{it is empirically true, is it formally rigorous ?}}
\end{align*}


Now, we bound $\| C\|^2$. We have 
\begin{align*}
    \| C\|^2 &= \sum_{s, s'}\frac{1}{\big\vert1 - e^{-2\alpha/K}e^{i(s-s')\pi/K}\big\vert^2}\\
    &=\sum_{s, s'}\frac{1}{\big(1-e^{-2\alpha/K}\cos(\frac{(s-s')\pi}{K}\big)^2 + e^{-4\alpha/K}\sin^2(\frac{(s-s')\pi}{K})}\\
    &= \sum_{s, s'}\frac{1}{\big(1 + e^{-4\alpha/K} - 2e^{-2\alpha/K}\cos(\frac{(s-s')\pi}{K})\big)}\\
    &=\sum_{s, s'}\frac{1}{1 + e^{-4\alpha/K} - 2e^{-2\alpha/K}\big(1 - \frac{(s-s')^2\pi}{2K^2} + o(\frac{1}{K^2})\big)}\\
    &= \sum_{s, s'}\frac{1}{2 - \frac{4\alpha}{K} + \frac{8\alpha}{K^2} + o(\frac{1}{K^2}) - 2\big[1 - \frac{(s-s')^2\pi^2}{2K^2}-\frac{2\alpha}{K}+\frac{2\alpha^2}{K^2}+o(\frac{1}{K^2})\big]}\\
    &= \sum_{s, s'}\frac{K^2}{4\alpha^2 + (s-s')^2\pi^2 + o(1)}\\
    &= K^2\sum_{\Delta=-2T}^{2T}\frac{2T + 1}{4\alpha^2 + \Delta^2 + o(1)}\\
    &=O(K^2T)
\end{align*}

So $\| C^{-1}\|^2 = O(\frac{1}{K^2T})$. \alex{this is true only if the condition number is bounded}

Now we bound $\| (KM)\|^2$. We recall that $M(s, s') = \frac{1}{2\alpha + i(s-s')\pi}$. So 
\begin{align*}
    \| KM \|^2 &= K^2\sum_{s, s'}\big\vert \frac{1}{2\alpha + i(s-s')\pi}\big\vert^2\\
    &= K^2\sum_{s, s'}\frac{1}{4\alpha^2 + (s-s')^2\pi^2}\\
    &= O(K^2T).
\end{align*}

Therefore, 
\[
 \big\vert\big[\big( C^{-1} - \frac{M^{-1}}{K}\big)\bar{a}^K\big]_u\big\vert = O\big(\frac{1}{K^2}\big).
\]

We can finally conclude that 
\[
b_s= \big(\frac{M^{-1}_{\infty}}{K}\bar{a}_\infty^K\big)_s= \frac{e^{-\alpha}(e^{2\alpha} - e^{-2\alpha})}{2K}(-1)^s + O\big(\frac{1}{K^2}\big).
\]
\end{proof}
